A VLT/NACO Study of Star Formation in the Massive Embedded Cluster RCW 38

We present adaptive optics (AO) near-infrared (JHKs) observations of the deeply embedded massive cluster RCW 38 using NACO on the VLT. Narrowband AO observations centered at wavelengths of 1.28, 2.12, and 2.17 micron were also obtained. The area covered by these observations is about 0.5 pc square, centered on the O star RCW 38 IRS2. We use the JHKs colors to identify young stars with infrared excess. Through a detailed comparison to a nearby control field, we find that most of the 337 stars detected in all three infrared bands are cluster members (~317), with essentially no contamination due to background or foreground sources. Five sources have colors suggestive of deeply embedded protostars, while 53 sources are detected at Ks only; their spatial distribution with respect to the extinction suggests they are highly reddened cluster members. Detectable Ks-band excess is found toward 29 +/- 3 % of the stars. For comparison to a similar area of Orion observed in the near-infrared, mass and extinction cuts are applied, and the excess fractions redetermined. The resulting excesses are then 25 +/- 5 % for RCW 38, and 42 +/- 8 % for Orion. RCW 38 IRS2 is shown to be a massive star binary with a projected separation of ~500 AU. Two regions of molecular hydrogen emission are revealed through the 2.12 micron imaging. One shows a morphology suggestive of a protostellar jet, and is clearly associated with a star only detected at H and Ks, previously identified as a highly obscured X-ray source. Three spatially extended cometary-like objects, suggestive of photoevaporating disks, are identified, but only one is clearly directly influenced by RCW 38 IRS2. A King profile provides a reasonable fit to the cluster radial density profile and a nearest neighbor distance analysis shows essentially no sub-clustering.

==> tab1.tex <==
\begin{deluxetable}{lllccccccl}
%\tablewidth{0pt}
\tablewidth{519.03049pt}
\tablecaption{Infrared Photometry of sources detected with magnitude
uncertainties $<$ 0.2.}
\tablehead{
\colhead{Source Number} & \colhead{R.A. (J2000)} & \colhead{Dec. (J2000)} &
\colhead{$J$} & \colhead {$J_{\rm err}$}  &
\colhead{$H$} & \colhead {$H_{\rm err}$}  &
\colhead{$K_s$} & \colhead {$(K_s)_{\rm err}$}  & 
\colhead{Notes} \\
}
\startdata
1 & 8 59 2.49 & -47 30 20.7 & \nodata & \nodata & \nodata & \nodata & 14.09 & 0.06 &  \\
2 & 8 59 2.50 & -47 30 52.6 & \nodata & \nodata & \nodata & \nodata & 15.02 & 0.09 &  \\
3 & 8 59 2.55 & -47 30 39.9 & \nodata & \nodata & \nodata & \nodata & 14.41 & 0.06 &  \\
4 & 8 59 2.56 & -47 30 46.2 & \nodata & \nodata & \nodata & \nodata & 12.08 & 0.02 &  \\
5 & 8 59 2.57 & -47 30 53.5 & \nodata & \nodata & \nodata & \nodata & 13.09 & 0.03 &  \\
6 & 8 59 2.60 & -47 30 31.7 & \nodata & \nodata & \nodata & \nodata & 13.35 & 0.04 &  \\
7 & 8 59 2.62 & -47 30 35.2 & \nodata & \nodata & \nodata & \nodata & 12.86 & 0.03 &  \\
8 & 8 59 2.63 & -47 30 28.7 & \nodata & \nodata & \nodata & \nodata & 15.07 & 0.08 &  \\
9 & 8 59 2.66 & -47 30 42.3 & \nodata & \nodata & \nodata & \nodata & 13.52 & 0.04 &  \\
10 & 8 59 2.67 & -47 30 57.4 & \nodata & \nodata & \nodata & \nodata & 15.68 & 0.14 &  \\
11 & 8 59 2.67 & -47 30 21.1 & \nodata & \nodata & \nodata & \nodata & 14.83 & 0.08 &  \\
12 & 8 59 2.74 & -47 30 43.4 & 17.72 & 0.07 & \nodata & \nodata & 15.32 & 0.09 &  \\
13 & 8 59 2.76 & -47 30 53.8 & 17.28 & 0.13 & \nodata & \nodata & 14.95 & 0.07 &  \\
14 & 8 59 2.78 & -47 30 46.8 & 14.97 & 0.02 & 13.61 & 0.02 & 12.65 & 0.03 & e \\
15 & 8 59 2.83 & -47 30 34.0 & \nodata & \nodata & \nodata & \nodata & 16.49 & 0.15 &  \\
16 & 8 59 2.89 & -47 31 6.5 & \nodata & \nodata & \nodata & \nodata & 15.25 & 0.10 &  \\
17 & 8 59 2.91 & -47 30 30.8 & 16.97 & 0.05 & 15.11 & 0.05 & 13.83 & 0.04 & e \\
18 & 8 59 2.92 & -47 31 2.1 & 15.01 & 0.02 & 13.44 & 0.02 & 12.36 & 0.02 & e \\
19 & 8 59 2.93 & -47 30 54.1 & 12.27 & 0.01 & 10.51 & 0.01 & 9.81 & 0.01 &  \\
20 & 8 59 2.93 & -47 30 54.1 & 12.14 & 0.02 & \nodata & \nodata & \nodata & \nodata &  \\
21 & 8 59 2.97 & -47 30 39.8 & 15.10 & 0.02 & 13.71 & 0.02 & 12.85 & 0.03 & e \\
22 & 8 59 2.98 & -47 30 51.7 & 17.88 & 0.10 & 15.90 & 0.06 & 14.12 & 0.05 & p \\
23 & 8 59 2.99 & -47 31 0.9 & \nodata & \nodata & 16.78 & 0.10 & 15.49 & 0.10 &  \\
24 & 8 59 3.00 & -47 30 44.4 & 16.25 & 0.03 & 13.54 & 0.02 & 11.00 & 0.01 & p \\
25 & 8 59 3.02 & -47 30 35.6 & 14.88 & 0.02 & 12.67 & 0.01 & 11.47 & 0.01 &  \\
26 & 8 59 3.03 & -47 31 3.8 & \nodata & \nodata & 14.40 & 0.03 & 13.39 & 0.04 &  \\
27 & 8 59 3.04 & -47 30 32.9 & 17.02 & 0.05 & 15.09 & 0.04 & 14.04 & 0.05 &  \\
28 & 8 59 3.05 & -47 30 42.5 & 15.55 & 0.02 & 13.61 & 0.02 & 12.73 & 0.03 &  \\
29 & 8 59 3.07 & -47 30 34.4 & 16.92 & 0.05 & 15.02 & 0.04 & 13.80 & 0.04 & e \\
30 & 8 59 3.12 & -47 30 11.2 & \nodata & \nodata & \nodata & \nodata & 16.23 & 0.17 &  \\
31 & 8 59 3.13 & -47 30 42.6 & \nodata & \nodata & 17.99 & 0.18 & \nodata & \nodata &  \\
32 & 8 59 3.17 & -47 30 11.3 & \nodata & \nodata & \nodata & \nodata & 14.37 & 0.06 &  \\
33 & 8 59 3.18 & -47 30 48.4 & 17.42 & 0.05 & 15.52 & 0.05 & 14.66 & 0.06 &  \\
34 & 8 59 3.24 & -47 30 42.6 & 17.74 & 0.06 & 16.20 & 0.07 & \nodata & \nodata &  \\
35 & 8 59 3.29 & -47 30 59.9 & 17.85 & 0.07 & 15.90 & 0.06 & 14.80 & 0.07 &  \\
36 & 8 59 3.29 & -47 30 49.1 & 17.54 & 0.06 & 15.87 & 0.06 & 14.83 & 0.06 &  \\
37 & 8 59 3.35 & -47 30 49.1 & 17.08 & 0.05 & 15.49 & 0.05 & 14.73 & 0.06 &  \\
38 & 8 59 3.35 & -47 30 45.4 & 16.55 & 0.04 & 14.92 & 0.04 & 14.10 & 0.05 &  \\
39 & 8 59 3.37 & -47 30 45.0 & 18.73 & 0.10 & 17.21 & 0.11 & 16.14 & 0.12 &  \\
40 & 8 59 3.38 & -47 30 51.7 & 19.62 & 0.16 & 16.64 & 0.08 & 14.70 & 0.06 & e \\
41 & 8 59 3.40 & -47 30 59.1 & 16.85 & 0.04 & 15.01 & 0.04 & 14.10 & 0.05 &  \\
42 & 8 59 3.40 & -47 30 41.0 & 19.25 & 0.14 & 17.71 & 0.14 & 16.59 & 0.16 &  \\
43 & 8 59 3.41 & -47 30 58.5 & 17.49 & 0.06 & 15.76 & 0.06 & 14.92 & 0.07 &  \\
44 & 8 59 3.42 & -47 30 28.2 & \nodata & \nodata & 17.51 & 0.13 & 16.09 & 0.12 &  \\
45 & 8 59 3.45 & -47 30 50.7 & 16.37 & 0.03 & 14.47 & 0.03 & 13.34 & 0.03 &  \\
46 & 8 59 3.50 & -47 30 56.7 & 18.69 & 0.11 & 17.04 & 0.11 & 16.12 & 0.12 &  \\
47 & 8 59 3.52 & -47 30 58.1 & 13.81 & 0.01 & 12.11 & 0.01 & 11.21 & 0.01 &  \\
48 & 8 59 3.53 & -47 31 8.1 & \nodata & \nodata & 15.93 & 0.07 & 14.91 & 0.08 &  \\
49 & 8 59 3.56 & -47 31 2.0 & 17.13 & 0.05 & 15.33 & 0.05 & 14.20 & 0.05 & e \\
50 & 8 59 3.59 & -47 30 34.9 & 19.31 & 0.15 & 17.39 & 0.12 & 16.04 & 0.11 &  \\
51 & 8 59 3.59 & -47 30 30.4 & 16.74 & 0.04 & 14.98 & 0.04 & 14.21 & 0.05 &  \\
52 & 8 59 3.59 & -47 30 32.3 & 16.18 & 0.03 & 14.29 & 0.03 & 13.25 & 0.03 &  \\
53 & 8 59 3.61 & -47 30 53.4 & 18.11 & 0.08 & 16.30 & 0.07 & 15.25 & 0.08 &  \\
54 & 8 59 3.61 & -47 31 6.1 & \nodata & \nodata & 17.84 & 0.18 & 15.96 & 0.12 &  \\
55 & 8 59 3.63 & -47 31 8.1 & \nodata & \nodata & 16.40 & 0.09 & 14.87 & 0.07 &  \\
56 & 8 59 3.64 & -47 30 34.0 & 16.88 & 0.04 & 15.20 & 0.04 & 14.43 & 0.05 &  \\
57 & 8 59 3.64 & -47 30 28.4 & 17.75 & 0.06 & 15.75 & 0.05 & 14.54 & 0.06 &  \\
58 & 8 59 3.64 & -47 30 56.3 & 15.18 & 0.02 & 13.19 & 0.02 & 11.99 & 0.02 & e \\
59 & 8 59 3.64 & -47 30 17.4 & 16.65 & 0.04 & 14.88 & 0.04 & 14.02 & 0.05 &  \\
60 & 8 59 3.65 & -47 30 40.0 & 18.03 & 0.12 & 15.06 & 0.04 & 12.89 & 0.03 & e \\
61 & 8 59 3.66 & -47 31 2.6 & 18.44 & 0.10 & 16.49 & 0.08 & 15.11 & 0.08 & e \\
62 & 8 59 3.69 & -47 30 52.4 & 17.21 & 0.05 & 15.21 & 0.04 & 13.91 & 0.04 & e \\
63 & 8 59 3.69 & -47 30 24.0 & 18.58 & 0.19 & 16.81 & 0.11 & 15.83 & 0.14 &  \\
64 & 8 59 3.72 & -47 30 39.2 & 16.79 & 0.04 & 14.86 & 0.04 & 13.72 & 0.04 &  \\
65 & 8 59 3.72 & -47 30 40.2 & 15.34 & 0.02 & 13.52 & 0.02 & 12.64 & 0.02 &  \\
66 & 8 59 3.73 & -47 30 50.3 & 19.23 & 0.13 & 16.52 & 0.08 & 15.05 & 0.07 &  \\
67 & 8 59 3.75 & -47 30 25.0 & \nodata & \nodata & 17.33 & 0.15 & 16.01 & 0.15 &  \\
68 & 8 59 3.76 & -47 30 38.1 & \nodata & \nodata & 17.99 & 0.17 & 16.58 & 0.15 &  \\
69 & 8 59 3.76 & -47 31 8.5 & 16.91 & 0.05 & 14.79 & 0.04 & 13.72 & 0.04 &  \\
70 & 8 59 3.76 & -47 31 8.5 & 16.99 & 0.05 & \nodata & \nodata & \nodata & \nodata &  \\
71 & 8 59 3.77 & -47 30 41.0 & 17.94 & 0.13 & 15.72 & 0.07 & 14.42 & 0.08 &  \\
72 & 8 59 3.77 & -47 30 38.1 & \nodata & \nodata & 17.92 & 0.17 & 16.62 & 0.16 &  \\
73 & 8 59 3.80 & -47 30 50.9 & 17.65 & 0.06 & 15.70 & 0.05 & 14.73 & 0.06 &  \\
74 & 8 59 3.80 & -47 30 27.8 & 16.98 & 0.04 & 14.78 & 0.03 & 13.53 & 0.03 &  \\
75 & 8 59 3.81 & -47 30 48.2 & 14.49 & 0.01 & 12.96 & 0.01 & 12.21 & 0.02 &  \\
76 & 8 59 3.86 & -47 30 51.2 & \nodata & \nodata & \nodata & \nodata & 16.49 & 0.14 &  \\
77 & 8 59 3.88 & -47 31 8.9 & 17.38 & 0.06 & \nodata & \nodata & 13.71 & 0.04 &  \\
78 & 8 59 3.90 & -47 31 4.5 & 16.41 & 0.04 & 14.00 & 0.03 & 12.33 & 0.02 & e \\
79 & 8 59 3.91 & -47 30 30.3 & 18.24 & 0.08 & 16.42 & 0.07 & 15.39 & 0.08 &  \\
80 & 8 59 3.91 & -47 30 46.4 & 18.45 & 0.13 & 16.76 & 0.11 & 15.02 & 0.09 & p \\
81 & 8 59 3.91 & -47 30 38.5 & \nodata & \nodata & \nodata & \nodata & 17.18 & 0.19 &  \\
82 & 8 59 3.93 & -47 30 17.7 & 17.78 & 0.07 & 16.01 & 0.07 & 15.03 & 0.07 &  \\
83 & 8 59 3.94 & -47 30 56.5 & 17.48 & 0.06 & 15.64 & 0.05 & 14.75 & 0.06 &  \\
84 & 8 59 3.95 & -47 31 1.5 & \nodata & \nodata & 18.36 & 0.19 & \nodata & \nodata &  \\
85 & 8 59 3.96 & -47 30 39.7 & 18.04 & 0.11 & 16.69 & 0.09 & 15.51 & 0.10 & e \\
86 & 8 59 4.01 & -47 30 57.2 & 17.10 & 0.05 & 15.01 & 0.04 & 13.83 & 0.04 &  \\
87 & 8 59 4.01 & -47 30 56.4 & \nodata & \nodata & \nodata & \nodata & 15.89 & 0.13 &  \\
88 & 8 59 4.02 & -47 30 59.3 & 17.76 & 0.06 & 15.83 & 0.06 & 14.58 & 0.06 & e \\
89 & 8 59 4.03 & -47 30 52.9 & 15.39 & 0.02 & 13.33 & 0.02 & 12.04 & 0.02 & e \\
90 & 8 59 4.03 & -47 30 55.2 & 16.81 & 0.04 & 14.86 & 0.04 & 13.75 & 0.04 &  \\
91 & 8 59 4.04 & -47 30 32.7 & \nodata & \nodata & 18.40 & 0.19 & \nodata & \nodata &  \\
92 & 8 59 4.04 & -47 30 55.5 & 16.08 & 0.03 & 14.11 & 0.03 & 12.94 & 0.03 &  \\
93 & 8 59 4.04 & -47 30 21.2 & 19.42 & 0.16 & 16.96 & 0.10 & 15.47 & 0.09 &  \\
94 & 8 59 4.05 & -47 30 34.5 & 15.27 & 0.02 & 13.57 & 0.02 & 12.78 & 0.02 &  \\
95 & 8 59 4.06 & -47 30 13.2 & \nodata & \nodata & 16.95 & 0.11 & 15.56 & 0.10 &  \\
96 & 8 59 4.10 & -47 30 40.4 & 18.21 & 0.10 & 16.11 & 0.06 & 14.77 & 0.06 &  \\
97 & 8 59 4.10 & -47 30 47.3 & 17.47 & 0.16 & 15.44 & 0.08 & 13.88 & 0.07 & e \\
98 & 8 59 4.11 & -47 30 56.8 & 18.91 & 0.12 & 17.08 & 0.10 & 15.84 & 0.10 &  \\
99 & 8 59 4.11 & -47 30 59.2 & 17.84 & 0.06 & 15.97 & 0.06 & 15.01 & 0.07 &  \\
100 & 8 59 4.19 & -47 30 34.8 & \nodata & \nodata & \nodata & \nodata & 16.55 & 0.19 &  \\
101 & 8 59 4.20 & -47 30 54.1 & \nodata & \nodata & 18.38 & 0.18 & \nodata & \nodata &  \\
102 & 8 59 4.20 & -47 30 51.7 & 16.66 & 0.06 & 14.78 & 0.04 & 13.87 & 0.05 &  \\
103 & 8 59 4.22 & -47 30 49.0 & 16.81 & 0.05 & 14.77 & 0.03 & 13.60 & 0.03 &  \\
104 & 8 59 4.22 & -47 30 60.0 & 16.16 & 0.03 & 14.15 & 0.03 & 13.02 & 0.03 &  \\
105 & 8 59 4.23 & -47 30 33.6 & \nodata & \nodata & 17.24 & 0.10 & 15.83 & 0.09 &  \\
106 & 8 59 4.25 & -47 30 12.2 & 17.44 & 0.06 & 15.52 & 0.06 & 14.58 & 0.06 &  \\
107 & 8 59 4.25 & -47 30 41.9 & \nodata & \nodata & \nodata & \nodata & 16.91 & 0.17 &  \\
108 & 8 59 4.25 & -47 30 13.5 & 17.42 & 0.06 & 15.57 & 0.06 & 14.69 & 0.07 &  \\
109 & 8 59 4.26 & -47 30 40.8 & 16.76 & 0.04 & 14.79 & 0.03 & 13.66 & 0.03 &  \\
110 & 8 59 4.28 & -47 30 39.5 & \nodata & \nodata & 18.00 & 0.15 & 17.04 & 0.16 &  \\
111 & 8 59 4.29 & -47 30 46.5 & 16.43 & 0.04 & 14.45 & 0.03 & 13.18 & 0.03 & e \\
112 & 8 59 4.31 & -47 30 44.7 & 18.30 & 0.12 & 16.32 & 0.07 & 14.93 & 0.07 & e \\
113 & 8 59 4.31 & -47 30 34.8 & 16.57 & 0.04 & 14.59 & 0.03 & 13.47 & 0.03 &  \\
114 & 8 59 4.32 & -47 30 47.4 & 16.98 & 0.05 & 15.01 & 0.04 & 13.75 & 0.04 & e \\
115 & 8 59 4.32 & -47 31 5.4 & 15.57 & 0.02 & 13.66 & 0.02 & 12.53 & 0.02 & e \\
116 & 8 59 4.33 & -47 30 27.3 & 18.69 & 0.10 & 17.20 & 0.10 & 15.88 & 0.10 & e \\
117 & 8 59 4.36 & -47 30 55.8 & 17.73 & 0.07 & 16.13 & 0.06 & 15.19 & 0.07 &  \\
118 & 8 59 4.36 & -47 30 45.6 & 19.42 & 0.18 & 17.52 & 0.12 & 16.22 & 0.12 &  \\
119 & 8 59 4.39 & -47 30 59.5 & 16.96 & 0.04 & 15.08 & 0.04 & 14.22 & 0.05 &  \\
120 & 8 59 4.39 & -47 30 48.0 & \nodata & \nodata & 17.78 & 0.14 & 16.76 & 0.16 &  \\
121 & 8 59 4.40 & -47 30 12.3 & \nodata & \nodata & 17.00 & 0.11 & 15.35 & 0.09 &  \\
122 & 8 59 4.40 & -47 30 46.2 & \nodata & \nodata & 17.70 & 0.13 & 16.25 & 0.12 &  \\
123 & 8 59 4.41 & -47 30 57.8 & 19.59 & 0.15 & 17.64 & 0.13 & 16.45 & 0.13 &  \\
124 & 8 59 4.43 & -47 30 56.0 & 13.31 & 0.01 & 11.41 & 0.01 & 10.47 & 0.01 &  \\
125 & 8 59 4.44 & -47 30 13.1 & 15.79 & 0.03 & 13.91 & 0.03 & 13.04 & 0.03 &  \\
126 & 8 59 4.44 & -47 30 58.5 & 18.16 & 0.07 & 16.08 & 0.06 & 14.80 & 0.06 &  \\
127 & 8 59 4.47 & -47 30 38.6 & 15.75 & 0.02 & 13.98 & 0.02 & 13.11 & 0.03 &  \\
128 & 8 59 4.48 & -47 30 32.7 & 18.62 & 0.13 & 16.68 & 0.08 & 15.58 & 0.09 &  \\
129 & 8 59 4.50 & -47 30 38.1 & \nodata & \nodata & 16.83 & 0.10 & 15.60 & 0.15 &  \\
130 & 8 59 4.50 & -47 30 41.7 & 18.26 & 0.08 & 16.55 & 0.07 & 15.75 & 0.09 &  \\
131 & 8 59 4.51 & -47 30 34.8 & 14.68 & 0.03 & 13.25 & 0.02 & 12.29 & 0.02 & e \\
132 & 8 59 4.52 & -47 30 26.2 & 17.60 & 0.06 & 15.90 & 0.06 & 15.03 & 0.07 &  \\
133 & 8 59 4.52 & -47 30 35.3 & 12.02 & 0.01 & 10.70 & 0.01 & 9.83 & 0.01 & e \\
134 & 8 59 4.53 & -47 31 1.8 & 19.63 & 0.16 & 17.69 & 0.14 & 16.45 & 0.13 &  \\
135 & 8 59 4.53 & -47 30 30.8 & 18.27 & 0.09 & 16.33 & 0.07 & 15.24 & 0.07 &  \\
136 & 8 59 4.53 & -47 30 57.3 & 18.86 & 0.10 & 16.53 & 0.08 & 15.19 & 0.07 &  \\
137 & 8 59 4.54 & -47 30 33.7 & 17.69 & 0.09 & 15.73 & 0.05 & 14.53 & 0.05 &  \\
138 & 8 59 4.54 & -47 30 40.6 & 17.06 & 0.08 & 15.01 & 0.04 & 13.81 & 0.04 &  \\
139 & 8 59 4.55 & -47 30 57.7 & \nodata & \nodata & 17.86 & 0.14 & 16.43 & 0.13 &  \\
140 & 8 59 4.56 & -47 30 34.3 & 17.62 & 0.07 & 16.32 & 0.07 & 15.44 & 0.08 &  \\
141 & 8 59 4.57 & -47 30 37.5 & 16.16 & 0.03 & 14.34 & 0.02 & 13.54 & 0.03 &  \\
142 & 8 59 4.58 & -47 30 35.2 & 15.06 & 0.03 & 14.00 & 0.03 & 13.35 & 0.03 &  \\
143 & 8 59 4.58 & -47 30 50.6 & 14.38 & 0.01 & 12.60 & 0.01 & 11.73 & 0.01 &  \\
144 & 8 59 4.59 & -47 30 53.7 & 18.78 & 0.10 & 16.40 & 0.07 & 14.54 & 0.05 & e \\
145 & 8 59 4.59 & -47 30 33.9 & 16.47 & 0.04 & 14.62 & 0.03 & 13.43 & 0.03 & e \\
146 & 8 59 4.60 & -47 30 47.4 & \nodata & \nodata & 17.81 & 0.17 & 16.66 & 0.18 &  \\
147 & 8 59 4.60 & -47 30 27.8 & 16.63 & 0.04 & 14.77 & 0.03 & 13.70 & 0.03 &  \\
148 & 8 59 4.60 & -47 30 40.4 & 15.60 & 0.02 & 13.65 & 0.02 & 12.53 & 0.02 &  \\
149 & 8 59 4.62 & -47 30 48.1 & 16.55 & 0.03 & 14.52 & 0.03 & 13.28 & 0.03 & e \\
150 & 8 59 4.62 & -47 30 52.3 & \nodata & \nodata & 18.59 & 0.19 & \nodata & \nodata &  \\
151 & 8 59 4.63 & -47 30 16.3 & 16.67 & 0.04 & 14.87 & 0.04 & 14.06 & 0.05 &  \\
152 & 8 59 4.64 & -47 30 28.0 & 15.52 & 0.02 & 13.43 & 0.02 & 11.96 & 0.02 & e \\
153 & 8 59 4.67 & -47 30 58.8 & 18.96 & 0.11 & 16.62 & 0.08 & 15.28 & 0.08 &  \\
154 & 8 59 4.67 & -47 30 52.5 & 17.60 & 0.05 & 15.49 & 0.04 & 14.15 & 0.04 & e \\
155 & 8 59 4.69 & -47 30 38.6 & \nodata & \nodata & 18.10 & 0.16 & 17.34 & 0.20 &  \\
156 & 8 59 4.70 & -47 30 48.7 & 15.82 & 0.02 & 13.90 & 0.02 & 12.72 & 0.02 & e \\
157 & 8 59 4.71 & -47 30 53.6 & 18.22 & 0.07 & 16.22 & 0.06 & 14.98 & 0.06 &  \\
158 & 8 59 4.73 & -47 30 42.0 & 18.36 & 0.08 & 16.57 & 0.07 & 15.59 & 0.08 &  \\
159 & 8 59 4.73 & -47 30 36.6 & 14.65 & 0.01 & 12.79 & 0.01 & 11.53 & 0.01 & e \\
160 & 8 59 4.74 & -47 30 16.4 & \nodata & \nodata & 17.58 & 0.13 & 15.53 & 0.09 &  \\
161 & 8 59 4.74 & -47 30 40.9 & 15.64 & 0.02 & 14.78 & 0.03 & 14.46 & 0.04 & x \\
162 & 8 59 4.78 & -47 30 32.3 & \nodata & \nodata & 18.29 & 0.16 & 17.13 & 0.16 &  \\
163 & 8 59 4.78 & -47 30 28.3 & 16.69 & 0.04 & 15.02 & 0.04 & 13.79 & 0.04 & e \\
164 & 8 59 4.79 & -47 31 7.0 & \nodata & \nodata & \nodata & \nodata & 16.83 & 0.17 &  \\
165 & 8 59 4.80 & -47 30 31.3 & 15.35 & 0.02 & 13.68 & 0.02 & 12.90 & 0.02 &  \\
166 & 8 59 4.81 & -47 30 20.9 & 15.98 & 0.03 & 14.11 & 0.03 & 13.06 & 0.03 &  \\
167 & 8 59 4.81 & -47 31 0.6 & \nodata & \nodata & 17.97 & 0.15 & 15.74 & 0.10 &  \\
168 & 8 59 4.83 & -47 30 54.2 & 16.45 & 0.03 & 14.47 & 0.03 & 13.49 & 0.03 &  \\
169 & 8 59 4.83 & -47 30 28.5 & 14.09 & 0.01 & 12.42 & 0.01 & 11.64 & 0.01 &  \\
170 & 8 59 4.85 & -47 31 1.3 & 17.94 & 0.07 & 15.92 & 0.06 & 14.94 & 0.07 &  \\
171 & 8 59 4.86 & -47 30 37.2 & 17.42 & 0.05 & 15.75 & 0.05 & 14.76 & 0.05 &  \\
172 & 8 59 4.87 & -47 30 54.9 & 20.16 & 0.20 & 18.11 & 0.15 & 16.97 & 0.16 &  \\
173 & 8 59 4.87 & -47 30 35.1 & 15.80 & 0.02 & 14.20 & 0.02 & 13.32 & 0.03 &  \\
174 & 8 59 4.87 & -47 30 53.5 & 19.14 & 0.12 & 17.23 & 0.10 & 16.16 & 0.11 &  \\
175 & 8 59 4.88 & -47 30 47.7 & 15.06 & 0.02 & 13.01 & 0.01 & 11.68 & 0.01 & e \\
176 & 8 59 4.88 & -47 30 48.7 & 16.08 & 0.03 & 14.16 & 0.02 & 13.20 & 0.03 &  \\
177 & 8 59 4.89 & -47 30 45.3 & 18.06 & 0.06 & 16.12 & 0.05 & 14.86 & 0.05 & e \\
178 & 8 59 4.89 & -47 30 50.6 & 19.02 & 0.11 & 17.15 & 0.09 & 16.12 & 0.10 &  \\
179 & 8 59 4.91 & -47 31 8.0 & \nodata & \nodata & \nodata & \nodata & 15.96 & 0.11 &  \\
180 & 8 59 4.95 & -47 30 53.0 & \nodata & \nodata & \nodata & \nodata & 17.39 & 0.19 &  \\
181 & 8 59 4.95 & -47 30 28.5 & 17.90 & 0.06 & 16.29 & 0.06 & 15.44 & 0.08 &  \\
182 & 8 59 4.97 & -47 30 27.8 & 17.13 & 0.04 & 15.46 & 0.04 & 14.48 & 0.05 &  \\
183 & 8 59 4.98 & -47 30 31.2 & 18.93 & 0.10 & 16.30 & 0.06 & 14.59 & 0.05 & e \\
184 & 8 59 4.98 & -47 30 35.0 & 17.33 & 0.05 & 15.59 & 0.04 & 14.55 & 0.05 &  \\
185 & 8 59 4.99 & -47 30 39.1 & \nodata & \nodata & 18.80 & 0.19 & 17.59 & 0.19 &  \\
186 & 8 59 5.00 & -47 30 44.2 & 17.57 & 0.05 & 15.67 & 0.04 & 14.45 & 0.04 & e \\
187 & 8 59 5.01 & -47 30 46.1 & 15.22 & 0.02 & 13.28 & 0.01 & 12.26 & 0.02 &  \\
188 & 8 59 5.01 & -47 30 57.8 & 17.54 & 0.06 & 14.69 & 0.03 & 13.08 & 0.03 &  \\
189 & 8 59 5.02 & -47 31 6.2 & \nodata & \nodata & \nodata & \nodata & 15.70 & 0.10 &  \\
190 & 8 59 5.05 & -47 30 26.1 & 16.25 & 0.03 & 14.54 & 0.03 & 13.72 & 0.03 &  \\
191 & 8 59 5.05 & -47 30 19.5 & \nodata & \nodata & \nodata & \nodata & 16.62 & 0.14 &  \\
192 & 8 59 5.06 & -47 30 47.2 & 15.61 & 0.02 & 13.81 & 0.02 & 12.92 & 0.02 &  \\
193 & 8 59 5.07 & -47 30 59.5 & 17.39 & 0.05 & 15.12 & 0.04 & 13.78 & 0.04 &  \\
194 & 8 59 5.07 & -47 30 53.1 & 17.50 & 0.05 & 15.28 & 0.04 & 13.99 & 0.04 &  \\
195 & 8 59 5.07 & -47 30 19.3 & 17.82 & 0.07 & 16.14 & 0.07 & 15.17 & 0.07 &  \\
196 & 8 59 5.08 & -47 31 4.8 & \nodata & \nodata & 17.99 & 0.16 & 15.58 & 0.09 &  \\
197 & 8 59 5.08 & -47 30 57.6 & 17.85 & 0.07 & 15.65 & 0.05 & 14.31 & 0.05 &  \\
198 & 8 59 5.09 & -47 30 30.7 & 16.14 & 0.03 & 14.32 & 0.02 & 13.15 & 0.03 & e \\
199 & 8 59 5.09 & -47 30 49.5 & 19.80 & 0.16 & 18.18 & 0.15 & 16.97 & 0.15 &  \\
200 & 8 59 5.10 & -47 30 48.9 & 18.67 & 0.09 & 16.76 & 0.07 & 15.60 & 0.08 &  \\
201 & 8 59 5.12 & -47 31 1.0 & 15.31 & 0.02 & 13.40 & 0.02 & 12.50 & 0.02 &  \\
202 & 8 59 5.12 & -47 30 59.1 & \nodata & \nodata & \nodata & \nodata & 16.11 & 0.11 &  \\
203 & 8 59 5.12 & -47 30 33.5 & 15.49 & 0.02 & 13.78 & 0.02 & 12.98 & 0.02 &  \\
204 & 8 59 5.13 & -47 30 41.6 & 17.99 & 0.06 & 16.30 & 0.06 & 15.44 & 0.07 &  \\
205 & 8 59 5.14 & -47 30 34.8 & 18.89 & 0.09 & \nodata & \nodata & \nodata & \nodata &  \\
206 & 8 59 5.14 & -47 31 2.2 & \nodata & \nodata & 17.18 & 0.11 & 15.34 & 0.08 &  \\
207 & 8 59 5.17 & -47 31 2.6 & \nodata & \nodata & \nodata & \nodata & 15.93 & 0.11 &  \\
208 & 8 59 5.19 & -47 30 37.3 & 18.77 & 0.09 & 17.24 & 0.09 & 16.26 & 0.10 &  \\
209 & 8 59 5.22 & -47 30 17.3 & 16.98 & 0.04 & 15.27 & 0.04 & 14.41 & 0.05 &  \\
210 & 8 59 5.23 & -47 30 29.5 & 16.65 & 0.03 & 14.96 & 0.03 & 14.09 & 0.04 &  \\
211 & 8 59 5.23 & -47 30 36.3 & 18.92 & 0.10 & 17.34 & 0.09 & 16.12 & 0.09 & e \\
212 & 8 59 5.24 & -47 30 27.9 & 19.63 & 0.14 & 18.16 & 0.15 & 17.16 & 0.16 &  \\
213 & 8 59 5.24 & -47 30 53.5 & 18.89 & 0.10 & 16.46 & 0.07 & 15.10 & 0.06 &  \\
214 & 8 59 5.25 & -47 30 42.5 & 15.32 & 0.02 & 13.02 & 0.01 & 11.33 & 0.01 & e \\
215 & 8 59 5.25 & -47 30 32.6 & 15.67 & 0.02 & 14.03 & 0.02 & 13.24 & 0.03 &  \\
216 & 8 59 5.26 & -47 30 33.3 & 18.67 & 0.09 & 17.10 & 0.09 & 16.25 & 0.10 &  \\
217 & 8 59 5.27 & -47 30 52.5 & 17.41 & 0.05 & 15.36 & 0.04 & 14.16 & 0.04 &  \\
218 & 8 59 5.28 & -47 30 59.1 & \nodata & \nodata & 17.64 & 0.13 & 15.38 & 0.08 &  \\
219 & 8 59 5.29 & -47 31 5.8 & 18.66 & 0.10 & 16.30 & 0.07 & 15.11 & 0.07 &  \\
220 & 8 59 5.31 & -47 30 57.1 & 17.61 & 0.06 & 15.69 & 0.05 & 14.70 & 0.05 &  \\
221 & 8 59 5.32 & -47 30 46.9 & 19.92 & 0.16 & 17.93 & 0.13 & 16.53 & 0.11 &  \\
222 & 8 59 5.37 & -47 31 0.4 & 18.21 & 0.07 & 16.10 & 0.06 & 15.12 & 0.07 &  \\
223 & 8 59 5.37 & -47 30 53.3 & 16.26 & 0.03 & 14.34 & 0.03 & 13.42 & 0.03 &  \\
224 & 8 59 5.38 & -47 30 31.7 & 17.35 & 0.05 & 15.77 & 0.05 & 14.95 & 0.06 &  \\
225 & 8 59 5.39 & -47 30 26.9 & 18.47 & 0.08 & 16.93 & 0.08 & 16.13 & 0.10 &  \\
226 & 8 59 5.40 & -47 30 54.9 & 14.73 & 0.02 & 13.51 & 0.02 & 12.75 & 0.02 & e \\
227 & 8 59 5.40 & -47 30 35.8 & 16.18 & 0.03 & 14.25 & 0.02 & 13.05 & 0.02 & e \\
228 & 8 59 5.40 & -47 31 7.2 & \nodata & \nodata & \nodata & \nodata & 15.70 & 0.10 &  \\
229 & 8 59 5.41 & -47 30 33.4 & 16.06 & 0.03 & 14.48 & 0.03 & 13.67 & 0.03 &  \\
230 & 8 59 5.41 & -47 30 47.9 & 16.62 & 0.03 & 14.79 & 0.03 & 13.88 & 0.03 &  \\
231 & 8 59 5.41 & -47 30 16.6 & 17.41 & 0.05 & 15.93 & 0.06 & 14.72 & 0.06 & e \\
232 & 8 59 5.42 & -47 30 38.2 & 16.03 & 0.03 & 14.06 & 0.02 & 12.88 & 0.02 & e \\
233 & 8 59 5.43 & -47 30 30.3 & 13.25 & 0.01 & 11.81 & 0.01 & 11.04 & 0.01 &  \\
234 & 8 59 5.44 & -47 30 21.5 & 17.60 & 0.06 & 15.94 & 0.06 & 14.90 & 0.06 &  \\
235 & 8 59 5.45 & -47 30 43.0 & 17.07 & 0.07 & 16.19 & 0.06 & 14.97 & 0.05 & x \\
236 & 8 59 5.46 & -47 30 32.0 & 15.51 & 0.02 & 13.94 & 0.02 & 13.08 & 0.02 &  \\
237 & 8 59 5.47 & -47 30 45.4 & 12.75 & 0.01 & 11.22 & 0.01 & 10.23 & 0.01 & e \\
238 & 8 59 5.47 & -47 30 40.0 & 16.96 & 0.07 & 16.29 & 0.09 & 15.84 & 0.08 & x \\
239 & 8 59 5.47 & -47 30 34.5 & 13.65 & 0.01 & 12.25 & 0.01 & 11.52 & 0.01 &  \\
240 & 8 59 5.48 & -47 30 41.9 & 14.24 & 0.02 & 12.57 & 0.01 & 11.76 & 0.01 &  \\
241 & 8 59 5.48 & -47 30 46.7 & 16.84 & 0.04 & 14.94 & 0.03 & 13.99 & 0.04 &  \\
242 & 8 59 5.49 & -47 30 40.0 & 16.56 & 0.06 & 16.24 & 0.11 & 15.49 & 0.10 & x \\
243 & 8 59 5.49 & -47 30 50.0 & 18.72 & 0.09 & 16.86 & 0.08 & 15.77 & 0.08 &  \\
244 & 8 59 5.53 & -47 30 53.9 & 18.70 & 0.09 & 16.46 & 0.07 & 15.25 & 0.07 &  \\
245 & 8 59 5.53 & -47 30 34.5 & 15.17 & 0.02 & 13.64 & 0.02 & 12.94 & 0.02 &  \\
246 & 8 59 5.53 & -47 30 36.0 & 12.62 & 0.01 & 11.16 & 0.01 & 10.19 & 0.01 & e \\
247 & 8 59 5.54 & -47 30 40.0 & 15.29 & 0.08 & 14.13 & 0.04 & 13.25 & 0.03 & e \\
248 & 8 59 5.55 & -47 31 1.3 & \nodata & \nodata & \nodata & \nodata & 17.13 & 0.18 &  \\
249 & 8 59 5.57 & -47 30 16.5 & 17.14 & 0.05 & 15.27 & 0.04 & 14.11 & 0.05 &  \\
250 & 8 59 5.58 & -47 30 48.8 & 17.86 & 0.06 & 15.87 & 0.05 & 14.93 & 0.05 &  \\
251 & 8 59 5.58 & -47 30 36.5 & \nodata & \nodata & \nodata & \nodata & 15.39 & 0.07 &  \\
252 & 8 59 5.59 & -47 30 56.1 & 18.78 & 0.09 & 16.78 & 0.08 & 15.73 & 0.09 &  \\
253 & 8 59 5.61 & -47 30 44.5 & 18.56 & 0.10 & 17.82 & 0.13 & 16.99 & 0.14 & x \\
254 & 8 59 5.61 & -47 30 38.3 & \nodata & \nodata & 17.06 & 0.09 & 16.40 & 0.13 &  \\
255 & 8 59 5.62 & -47 30 40.6 & 13.45 & 0.16 & \nodata & \nodata & \nodata & \nodata &  \\
256 & 8 59 5.63 & -47 30 43.7 & 15.61 & 0.02 & 13.86 & 0.02 & 13.07 & 0.02 &  \\
257 & 8 59 5.63 & -47 30 38.6 & 17.93 & 0.19 & 16.51 & 0.10 & 15.57 & 0.07 &  \\
258 & 8 59 5.63 & -47 30 38.3 & \nodata & \nodata & 17.04 & 0.12 & 16.28 & 0.12 &  \\
259 & 8 59 5.64 & -47 30 40.8 & 13.31 & 0.05 & \nodata & \nodata & \nodata & \nodata &  \\
260 & 8 59 5.64 & -47 30 23.9 & 18.11 & 0.07 & 16.40 & 0.07 & 15.40 & 0.08 &  \\
261 & 8 59 5.65 & -47 30 46.5 & 14.41 & 0.01 & 12.76 & 0.01 & 11.96 & 0.01 &  \\
262 & 8 59 5.65 & -47 30 54.2 & 16.64 & 0.03 & 14.49 & 0.03 & 13.29 & 0.03 &  \\
263 & 8 59 5.66 & -47 30 30.0 & 20.22 & 0.19 & \nodata & \nodata & \nodata & \nodata &  \\
264 & 8 59 5.67 & -47 30 51.4 & \nodata & \nodata & 17.61 & 0.11 & 15.83 & 0.09 &  \\
265 & 8 59 5.68 & -47 30 41.9 & \nodata & \nodata & 15.17 & 0.05 & \nodata & \nodata &  \\
266 & 8 59 5.70 & -47 31 5.2 & \nodata & \nodata & 18.30 & 0.19 & 15.62 & 0.09 &  \\
267 & 8 59 5.70 & -47 30 33.4 & 18.85 & 0.10 & \nodata & \nodata & \nodata & \nodata &  \\
268 & 8 59 5.71 & -47 30 46.8 & 18.71 & 0.11 & 17.20 & 0.09 & 16.23 & 0.10 &  \\
269 & 8 59 5.72 & -47 30 52.7 & 16.82 & 0.04 & 14.72 & 0.03 & 13.72 & 0.03 &  \\
270 & 8 59 5.72 & -47 30 50.2 & 16.07 & 0.03 & 14.10 & 0.02 & 13.16 & 0.02 &  \\
271 & 8 59 5.73 & -47 30 30.1 & 19.00 & 0.10 & 16.82 & 0.08 & 15.55 & 0.08 &  \\
272 & 8 59 5.74 & -47 30 44.6 & 15.16 & 0.02 & 13.36 & 0.01 & 12.50 & 0.02 &  \\
273 & 8 59 5.75 & -47 30 28.7 & 16.42 & 0.03 & 14.81 & 0.03 & 14.11 & 0.04 &  \\
274 & 8 59 5.75 & -47 30 46.2 & 18.36 & 0.08 & 16.30 & 0.06 & 15.01 & 0.06 &  \\
275 & 8 59 5.75 & -47 30 51.7 & 18.33 & 0.07 & 16.29 & 0.06 & 15.29 & 0.07 &  \\
276 & 8 59 5.77 & -47 30 15.4 & 18.63 & 0.10 & 16.83 & 0.09 & 15.73 & 0.10 &  \\
277 & 8 59 5.77 & -47 30 33.9 & 19.77 & 0.15 & 18.70 & 0.18 & 17.69 & 0.20 &  \\
278 & 8 59 5.78 & -47 31 4.9 & \nodata & \nodata & \nodata & \nodata & 16.43 & 0.14 &  \\
279 & 8 59 5.78 & -47 30 40.8 & 16.22 & 0.09 & 15.70 & 0.10 & 15.02 & 0.08 & x \\
280 & 8 59 5.80 & -47 30 25.0 & 18.02 & 0.07 & 16.40 & 0.07 & 15.45 & 0.08 &  \\
281 & 8 59 5.81 & -47 30 48.5 & 18.48 & 0.08 & 16.75 & 0.07 & 15.74 & 0.08 &  \\
282 & 8 59 5.82 & -47 30 19.5 & 19.34 & 0.13 & 17.61 & 0.13 & 16.47 & 0.13 &  \\
283 & 8 59 5.82 & -47 30 32.4 & 19.94 & 0.17 & 18.57 & 0.18 & 17.51 & 0.19 &  \\
284 & 8 59 5.83 & -47 30 18.0 & 17.01 & 0.04 & 14.92 & 0.04 & 13.63 & 0.04 & e \\
285 & 8 59 5.83 & -47 30 36.6 & 16.40 & 0.03 & 14.84 & 0.03 & 13.73 & 0.03 & e \\
286 & 8 59 5.83 & -47 30 36.4 & 16.31 & 0.03 & 14.56 & 0.03 & 13.55 & 0.03 &  \\
287 & 8 59 5.84 & -47 30 47.1 & 15.88 & 0.02 & 14.05 & 0.02 & 13.07 & 0.02 &  \\
288 & 8 59 5.84 & -47 30 49.5 & 19.15 & 0.11 & 17.22 & 0.09 & 15.90 & 0.09 & e \\
289 & 8 59 5.85 & -47 31 6.2 & \nodata & \nodata & \nodata & \nodata & 16.57 & 0.15 &  \\
290 & 8 59 5.86 & -47 30 50.2 & 17.83 & 0.06 & 15.76 & 0.05 & 14.55 & 0.05 &  \\
291 & 8 59 5.86 & -47 30 39.8 & \nodata & \nodata & \nodata & \nodata & 15.26 & 0.08 &  \\
292 & 8 59 5.87 & -47 31 4.9 & \nodata & \nodata & 17.70 & 0.14 & 15.54 & 0.09 &  \\
293 & 8 59 5.87 & -47 30 47.4 & 17.40 & 0.05 & 15.61 & 0.04 & 14.63 & 0.05 &  \\
294 & 8 59 5.88 & -47 30 42.9 & \nodata & \nodata & 17.64 & 0.14 & 16.49 & 0.11 &  \\
295 & 8 59 5.88 & -47 30 40.9 & 16.37 & 0.04 & 14.54 & 0.03 & 13.70 & 0.03 &  \\
296 & 8 59 5.88 & -47 30 30.8 & 14.05 & 0.01 & 12.49 & 0.01 & 11.72 & 0.01 &  \\
297 & 8 59 5.89 & -47 30 40.0 & 16.21 & 0.03 & 14.65 & 0.03 & 13.58 & 0.03 & e \\
298 & 8 59 5.89 & -47 30 40.9 & 16.71 & 0.06 & 14.95 & 0.03 & 14.05 & 0.04 &  \\
299 & 8 59 5.92 & -47 30 26.7 & 18.19 & 0.07 & 16.69 & 0.08 & 15.71 & 0.08 &  \\
300 & 8 59 5.92 & -47 30 32.6 & 15.88 & 0.02 & 13.96 & 0.02 & 12.65 & 0.02 & e \\
301 & 8 59 5.92 & -47 30 54.6 & 16.40 & 0.03 & 14.42 & 0.03 & 13.46 & 0.03 &  \\
302 & 8 59 5.93 & -47 30 42.3 & 15.77 & 0.02 & 14.07 & 0.02 & 13.28 & 0.02 &  \\
303 & 8 59 5.93 & -47 30 44.9 & 18.46 & 0.08 & 16.84 & 0.08 & 16.08 & 0.09 &  \\
304 & 8 59 5.93 & -47 30 29.9 & 16.74 & 0.04 & 15.02 & 0.03 & 14.07 & 0.04 &  \\
305 & 8 59 5.95 & -47 30 45.0 & 17.84 & 0.06 & 15.86 & 0.05 & 14.72 & 0.05 &  \\
306 & 8 59 5.96 & -47 30 34.6 & 18.31 & 0.08 & 16.82 & 0.08 & 15.77 & 0.08 & e \\
307 & 8 59 5.98 & -47 30 39.6 & 18.64 & 0.12 & 17.35 & 0.11 & 16.37 & 0.15 &  \\
308 & 8 59 5.98 & -47 30 38.6 & 16.17 & 0.03 & 14.22 & 0.02 & 12.98 & 0.02 & e \\
309 & 8 59 5.99 & -47 30 14.8 & \nodata & \nodata & 18.08 & 0.17 & \nodata & \nodata &  \\
310 & 8 59 5.99 & -47 30 37.3 & 16.95 & 0.04 & 15.24 & 0.04 & 14.20 & 0.04 &  \\
311 & 8 59 6.00 & -47 30 12.1 & \nodata & \nodata & 17.84 & 0.17 & 16.65 & 0.19 &  \\
312 & 8 59 6.01 & -47 30 36.3 & 18.11 & 0.11 & 16.57 & 0.07 & 15.43 & 0.07 & e \\
313 & 8 59 6.03 & -47 30 52.3 & 16.67 & 0.04 & 14.69 & 0.03 & 13.67 & 0.03 &  \\
314 & 8 59 6.04 & -47 30 34.6 & 17.48 & 0.06 & 15.94 & 0.05 & 14.80 & 0.05 & e \\
315 & 8 59 6.04 & -47 30 20.8 & 16.02 & 0.03 & 14.04 & 0.02 & 12.85 & 0.02 & e \\
316 & 8 59 6.07 & -47 30 44.8 & 17.76 & 0.06 & 15.74 & 0.05 & 14.33 & 0.04 & e \\
317 & 8 59 6.07 & -47 30 34.6 & 15.98 & 0.03 & 14.35 & 0.03 & 13.61 & 0.03 &  \\
318 & 8 59 6.08 & -47 31 1.2 & 18.56 & 0.09 & 15.61 & 0.05 & 14.02 & 0.04 &  \\
319 & 8 59 6.09 & -47 31 0.4 & \nodata & \nodata & \nodata & \nodata & 17.36 & 0.20 &  \\
320 & 8 59 6.10 & -47 30 44.4 & 15.43 & 0.02 & 13.63 & 0.02 & 12.83 & 0.02 &  \\
321 & 8 59 6.11 & -47 30 32.1 & \nodata & \nodata & 16.44 & 0.07 & 15.78 & 0.09 &  \\
322 & 8 59 6.11 & -47 30 36.9 & 18.05 & 0.09 & 16.23 & 0.06 & 14.58 & 0.05 & p \\
323 & 8 59 6.11 & -47 30 39.7 & 17.97 & 0.07 & 16.03 & 0.05 & 14.98 & 0.05 &  \\
324 & 8 59 6.12 & -47 30 27.4 & 18.18 & 0.07 & 16.44 & 0.07 & 15.30 & 0.07 & e \\
325 & 8 59 6.13 & -47 30 44.0 & 17.86 & 0.06 & 16.55 & 0.07 & 15.52 & 0.07 & e \\
326 & 8 59 6.13 & -47 30 53.2 & 19.72 & 0.16 & 17.56 & 0.11 & 15.85 & 0.09 & e \\
327 & 8 59 6.13 & -47 30 35.4 & 12.09 & 0.01 & 10.73 & 0.01 & 9.78 & 0.01 & e \\
328 & 8 59 6.16 & -47 30 32.3 & 13.17 & 0.01 & 12.08 & 0.01 & 11.48 & 0.01 &  \\
329 & 8 59 6.16 & -47 30 24.5 & 19.12 & 0.12 & 17.52 & 0.12 & 16.16 & 0.11 & e \\
330 & 8 59 6.16 & -47 31 0.2 & \nodata & \nodata & \nodata & \nodata & 16.40 & 0.13 &  \\
331 & 8 59 6.17 & -47 30 44.2 & 16.31 & 0.05 & 15.09 & 0.05 & 14.06 & 0.04 & e \\
332 & 8 59 6.19 & -47 30 51.1 & 16.19 & 0.03 & 13.87 & 0.02 & 12.40 & 0.02 & e \\
333 & 8 59 6.19 & -47 30 44.4 & 13.82 & 0.01 & 12.52 & 0.01 & 11.81 & 0.01 &  \\
334 & 8 59 6.20 & -47 30 44.3 & \nodata & \nodata & 12.94 & 0.01 & \nodata & \nodata &  \\
335 & 8 59 6.21 & -47 30 34.7 & 17.17 & 0.05 & 15.85 & 0.06 & 14.84 & 0.05 & e \\
336 & 8 59 6.24 & -47 30 37.7 & 19.69 & 0.15 & 18.18 & 0.14 & 16.84 & 0.14 & e \\
337 & 8 59 6.24 & -47 30 25.9 & 15.35 & 0.02 & 13.69 & 0.02 & 12.88 & 0.02 &  \\
338 & 8 59 6.25 & -47 30 56.9 & 17.84 & 0.06 & 14.99 & 0.04 & 13.21 & 0.03 & e \\
339 & 8 59 6.25 & -47 30 44.6 & 17.59 & 0.05 & 16.02 & 0.05 & 15.06 & 0.06 &  \\
340 & 8 59 6.26 & -47 30 46.0 & 19.16 & 0.11 & 17.39 & 0.10 & 16.25 & 0.10 &  \\
341 & 8 59 6.27 & -47 31 7.4 & 16.26 & 0.03 & 13.16 & 0.02 & 11.38 & 0.01 &  \\
342 & 8 59 6.29 & -47 31 7.0 & 17.46 & 0.06 & 14.28 & 0.03 & 12.46 & 0.02 &  \\
343 & 8 59 6.30 & -47 30 42.5 & 18.46 & 0.08 & 16.54 & 0.07 & 15.18 & 0.06 & e \\
344 & 8 59 6.34 & -47 30 37.7 & 18.43 & 0.09 & 16.64 & 0.07 & 15.62 & 0.08 &  \\
345 & 8 59 6.35 & -47 30 17.1 & 18.32 & 0.08 & 16.21 & 0.07 & 15.15 & 0.07 &  \\
346 & 8 59 6.36 & -47 30 30.8 & 15.31 & 0.02 & 13.41 & 0.02 & 12.27 & 0.02 & e \\
347 & 8 59 6.36 & -47 30 50.7 & 17.99 & 0.06 & 15.71 & 0.05 & 14.34 & 0.04 &  \\
348 & 8 59 6.37 & -47 30 58.7 & \nodata & \nodata & 18.46 & 0.19 & 16.14 & 0.11 &  \\
349 & 8 59 6.37 & -47 30 55.6 & 18.53 & 0.09 & 16.25 & 0.06 & 14.96 & 0.06 &  \\
350 & 8 59 6.38 & -47 30 39.0 & 17.14 & 0.04 & 15.12 & 0.03 & 14.03 & 0.04 &  \\
351 & 8 59 6.39 & -47 30 46.4 & 19.25 & 0.11 & 17.48 & 0.10 & 16.26 & 0.10 &  \\
352 & 8 59 6.39 & -47 30 57.1 & 18.26 & 0.08 & 16.25 & 0.07 & 15.05 & 0.07 &  \\
353 & 8 59 6.40 & -47 30 43.8 & 19.40 & 0.12 & 17.60 & 0.11 & 16.13 & 0.10 & e \\
354 & 8 59 6.42 & -47 30 20.6 & 19.10 & 0.12 & 17.05 & 0.10 & 15.83 & 0.10 &  \\
355 & 8 59 6.42 & -47 30 37.3 & 14.77 & 0.01 & 13.14 & 0.01 & 12.37 & 0.02 &  \\
356 & 8 59 6.42 & -47 30 54.3 & 17.29 & 0.05 & 15.09 & 0.04 & 13.82 & 0.04 &  \\
357 & 8 59 6.43 & -47 30 16.9 & 17.71 & 0.06 & 15.75 & 0.06 & 14.61 & 0.06 &  \\
358 & 8 59 6.43 & -47 30 53.0 & 14.78 & 0.02 & 13.32 & 0.02 & 12.49 & 0.02 &  \\
359 & 8 59 6.43 & -47 30 33.0 & 17.28 & 0.05 & 15.31 & 0.04 & 14.01 & 0.04 & e \\
360 & 8 59 6.44 & -47 31 6.4 & \nodata & \nodata & \nodata & \nodata & 15.53 & 0.09 &  \\
361 & 8 59 6.45 & -47 30 36.8 & 17.08 & 0.04 & 15.10 & 0.04 & 13.67 & 0.03 & e \\
362 & 8 59 6.46 & -47 30 20.4 & \nodata & \nodata & 18.19 & 0.18 & 17.11 & 0.20 &  \\
363 & 8 59 6.48 & -47 30 28.1 & 19.53 & 0.14 & 17.72 & 0.12 & 16.76 & 0.14 &  \\
364 & 8 59 6.48 & -47 30 36.8 & 18.42 & 0.09 & 16.85 & 0.08 & 15.69 & 0.08 & e \\
365 & 8 59 6.48 & -47 30 43.0 & \nodata & \nodata & 18.65 & 0.18 & 17.58 & 0.19 &  \\
366 & 8 59 6.49 & -47 30 21.1 & 17.26 & 0.05 & 14.75 & 0.03 & 13.14 & 0.03 & e \\
367 & 8 59 6.52 & -47 30 34.1 & 16.56 & 0.03 & 14.59 & 0.03 & 13.46 & 0.03 &  \\
368 & 8 59 6.55 & -47 30 36.3 & 19.72 & 0.17 & 17.90 & 0.13 & 17.01 & 0.16 &  \\
369 & 8 59 6.56 & -47 30 43.0 & 19.58 & 0.14 & 17.56 & 0.11 & 15.96 & 0.09 & e \\
370 & 8 59 6.57 & -47 30 11.3 & \nodata & \nodata & \nodata & \nodata & 14.40 & 0.06 &  \\
371 & 8 59 6.59 & -47 30 59.7 & \nodata & \nodata & 17.03 & 0.10 & 15.36 & 0.08 &  \\
372 & 8 59 6.60 & -47 30 22.0 & 18.28 & 0.08 & 16.02 & 0.06 & 14.62 & 0.06 &  \\
373 & 8 59 6.61 & -47 30 54.3 & 18.30 & 0.08 & 16.22 & 0.06 & 14.91 & 0.06 &  \\
374 & 8 59 6.61 & -47 30 18.3 & 16.84 & 0.04 & 14.59 & 0.03 & 13.21 & 0.03 & e \\
375 & 8 59 6.61 & -47 30 23.2 & 19.24 & 0.13 & 16.87 & 0.09 & 15.55 & 0.09 &  \\
376 & 8 59 6.62 & -47 30 35.7 & 18.23 & 0.07 & 16.51 & 0.07 & 15.57 & 0.08 &  \\
377 & 8 59 6.62 & -47 30 38.1 & 18.79 & 0.10 & 16.84 & 0.08 & 15.73 & 0.08 &  \\
378 & 8 59 6.62 & -47 30 57.2 & \nodata & \nodata & 18.27 & 0.17 & 16.71 & 0.14 &  \\
379 & 8 59 6.62 & -47 30 49.8 & 19.29 & 0.12 & 16.64 & 0.07 & 14.98 & 0.06 &  \\
380 & 8 59 6.64 & -47 31 1.0 & \nodata & \nodata & 17.37 & 0.12 & 14.52 & 0.05 &  \\
381 & 8 59 6.65 & -47 30 36.4 & 18.75 & 0.09 & 17.09 & 0.09 & 16.12 & 0.10 &  \\
382 & 8 59 6.67 & -47 30 41.1 & 19.09 & 0.11 & 16.13 & 0.06 & 14.15 & 0.04 & e \\
383 & 8 59 6.67 & -47 30 29.8 & \nodata & \nodata & 17.79 & 0.13 & 16.10 & 0.10 &  \\
384 & 8 59 6.70 & -47 30 46.9 & 19.04 & 0.11 & 16.74 & 0.08 & 14.94 & 0.06 & e \\
385 & 8 59 6.70 & -47 30 53.3 & \nodata & \nodata & 17.67 & 0.13 & 16.25 & 0.11 &  \\
386 & 8 59 6.72 & -47 31 1.0 & \nodata & \nodata & \nodata & \nodata & 16.68 & 0.15 &  \\
387 & 8 59 6.74 & -47 30 55.1 & 17.51 & 0.05 & 15.13 & 0.04 & 13.77 & 0.04 &  \\
388 & 8 59 6.77 & -47 30 45.1 & 19.06 & 0.11 & 16.57 & 0.07 & 15.06 & 0.06 &  \\
389 & 8 59 6.78 & -47 30 20.9 & \nodata & \nodata & \nodata & \nodata & 16.71 & 0.16 &  \\
390 & 8 59 6.79 & -47 30 22.7 & \nodata & \nodata & 18.12 & 0.17 & 16.83 & 0.16 &  \\
391 & 8 59 6.79 & -47 30 37.4 & 18.90 & 0.11 & 17.10 & 0.09 & 15.96 & 0.09 &  \\
392 & 8 59 6.79 & -47 30 40.2 & 17.37 & 0.05 & 15.43 & 0.04 & 14.49 & 0.05 &  \\
393 & 8 59 6.79 & -47 30 20.1 & 17.87 & 0.07 & 15.69 & 0.05 & 14.44 & 0.05 &  \\
394 & 8 59 6.80 & -47 30 54.8 & 18.70 & 0.09 & 16.55 & 0.08 & 15.40 & 0.08 &  \\
395 & 8 59 6.80 & -47 30 36.8 & \nodata & \nodata & \nodata & \nodata & 17.24 & 0.17 &  \\
396 & 8 59 6.81 & -47 30 26.3 & 19.02 & 0.12 & 16.89 & 0.09 & 15.64 & 0.09 &  \\
397 & 8 59 6.81 & -47 30 19.5 & 19.30 & 0.14 & 17.53 & 0.13 & 16.49 & 0.14 &  \\
398 & 8 59 6.82 & -47 30 53.3 & \nodata & \nodata & 18.48 & 0.19 & 16.79 & 0.15 &  \\
399 & 8 59 6.86 & -47 30 39.2 & \nodata & \nodata & 18.04 & 0.14 & 17.00 & 0.16 &  \\
400 & 8 59 6.86 & -47 30 25.1 & 14.40 & 0.01 & 13.02 & 0.02 & 12.19 & 0.02 & e \\
401 & 8 59 6.89 & -47 31 2.1 & \nodata & \nodata & 16.07 & 0.06 & 13.58 & 0.04 &  \\
402 & 8 59 6.89 & -47 30 23.6 & \nodata & \nodata & \nodata & \nodata & 16.78 & 0.16 &  \\
403 & 8 59 6.90 & -47 30 46.3 & 20.08 & 0.19 & 17.71 & 0.12 & 16.36 & 0.12 &  \\
404 & 8 59 6.95 & -47 30 45.1 & 19.54 & 0.14 & 17.41 & 0.11 & 16.22 & 0.11 &  \\
405 & 8 59 6.97 & -47 30 32.6 & 18.50 & 0.08 & 16.39 & 0.07 & 15.35 & 0.07 &  \\
406 & 8 59 6.98 & -47 30 24.7 & 20.09 & 0.20 & 17.20 & 0.11 & 15.79 & 0.10 &  \\
407 & 8 59 6.99 & -47 30 23.4 & 14.58 & 0.02 & 12.18 & 0.01 & 10.41 & 0.01 & e \\
408 & 8 59 7.00 & -47 30 54.3 & 17.97 & 0.07 & 15.76 & 0.05 & 14.54 & 0.05 &  \\
409 & 8 59 7.03 & -47 30 29.5 & \nodata & \nodata & \nodata & \nodata & 16.98 & 0.16 &  \\
410 & 8 59 7.04 & -47 30 35.0 & \nodata & \nodata & 18.17 & 0.16 & 16.90 & 0.15 &  \\
411 & 8 59 7.05 & -47 30 17.1 & 17.91 & 0.07 & 15.70 & 0.06 & 14.52 & 0.06 &  \\
412 & 8 59 7.05 & -47 30 42.7 & 19.59 & 0.15 & 17.65 & 0.12 & 16.49 & 0.12 &  \\
413 & 8 59 7.07 & -47 30 23.4 & \nodata & \nodata & 16.57 & 0.09 & 15.06 & 0.08 &  \\
414 & 8 59 7.08 & -47 30 39.2 & 18.08 & 0.07 & 15.45 & 0.04 & 13.95 & 0.04 &  \\
415 & 8 59 7.08 & -47 30 39.8 & 19.52 & 0.15 & 17.43 & 0.11 & 16.32 & 0.12 &  \\
416 & 8 59 7.11 & -47 30 38.3 & 20.09 & 0.19 & 18.14 & 0.15 & 16.89 & 0.15 &  \\
417 & 8 59 7.11 & -47 30 48.0 & 15.86 & 0.02 & 13.38 & 0.02 & 11.88 & 0.02 & e \\
418 & 8 59 7.16 & -47 30 36.7 & 16.24 & 0.03 & 13.73 & 0.02 & 12.25 & 0.02 &  \\
419 & 8 59 7.17 & -47 30 34.2 & 20.00 & 0.18 & 17.64 & 0.12 & 16.28 & 0.11 &  \\
420 & 8 59 7.18 & -47 31 4.5 & \nodata & \nodata & \nodata & \nodata & 15.90 & 0.11 &  \\
421 & 8 59 7.21 & -47 30 52.7 & 18.72 & 0.10 & 16.53 & 0.08 & 15.43 & 0.08 &  \\
422 & 8 59 7.22 & -47 31 8.2 & \nodata & \nodata & 17.58 & 0.15 & 15.16 & 0.08 &  \\
423 & 8 59 7.25 & -47 30 51.1 & 19.08 & 0.11 & 16.80 & 0.09 & 15.49 & 0.08 &  \\
424 & 8 59 7.26 & -47 30 15.0 & 18.18 & 0.08 & 15.84 & 0.06 & 14.45 & 0.06 &  \\
425 & 8 59 7.35 & -47 30 45.8 & 15.92 & 0.03 & 13.80 & 0.02 & 12.73 & 0.02 &  \\
426 & 8 59 7.36 & -47 30 43.7 & 18.51 & 0.08 & 15.90 & 0.06 & 14.44 & 0.05 &  \\
427 & 8 59 7.38 & -47 30 57.9 & 18.66 & 0.10 & 16.06 & 0.06 & 14.49 & 0.06 &  \\
428 & 8 59 7.39 & -47 30 37.1 & 19.21 & 0.12 & 16.31 & 0.07 & 14.50 & 0.05 &  \\
429 & 8 59 7.40 & -47 30 54.5 & 17.92 & 0.07 & 15.60 & 0.05 & 14.40 & 0.05 &  \\
430 & 8 59 7.43 & -47 30 18.5 & 17.88 & 0.07 & 15.47 & 0.05 & 14.30 & 0.05 &  \\
431 & 8 59 7.46 & -47 30 40.8 & 19.03 & 0.11 & 16.55 & 0.08 & 14.82 & 0.06 & e \\
432 & 8 59 7.50 & -47 31 5.8 & \nodata & \nodata & \nodata & \nodata & 16.74 & 0.17 &  \\
433 & 8 59 7.51 & -47 30 49.3 & \nodata & \nodata & 17.76 & 0.14 & 16.51 & 0.14 &  \\
434 & 8 59 7.51 & -47 30 18.0 & \nodata & \nodata & 17.04 & 0.11 & 15.66 & 0.10 &  \\
435 & 8 59 7.58 & -47 30 46.3 & 18.30 & 0.08 & 15.98 & 0.06 & 14.91 & 0.06 &  \\
436 & 8 59 7.59 & -47 30 44.3 & 19.74 & 0.16 & 17.37 & 0.11 & 16.22 & 0.12 &  \\
437 & 8 59 7.59 & -47 30 52.3 & \nodata & \nodata & 17.65 & 0.14 & 16.44 & 0.14 &  \\
438 & 8 59 7.60 & -47 31 3.4 & \nodata & \nodata & 17.80 & 0.15 & 15.92 & 0.12 &  \\
439 & 8 59 7.62 & -47 30 53.3 & 19.37 & 0.15 & 17.19 & 0.11 & 15.94 & 0.11 &  \\
440 & 8 59 7.63 & -47 30 55.0 & \nodata & \nodata & 18.19 & 0.19 & 16.96 & 0.19 &  \\
441 & 8 59 7.69 & -47 30 44.6 & 17.68 & 0.06 & 15.24 & 0.04 & 14.06 & 0.04 &  \\
442 & 8 59 7.70 & -47 30 46.3 & \nodata & \nodata & 18.00 & 0.15 & 16.83 & 0.16 &  \\
443 & 8 59 7.71 & -47 30 53.9 & 18.29 & 0.09 & 16.06 & 0.06 & 15.06 & 0.07 &  \\
444 & 8 59 7.73 & -47 30 58.8 & \nodata & \nodata & 17.78 & 0.16 & 16.62 & 0.18 &  \\
445 & 8 59 7.74 & -47 31 0.2 & \nodata & \nodata & 18.23 & 0.19 & 16.67 & 0.17 &  \\
446 & 8 59 7.74 & -47 31 4.0 & \nodata & \nodata & 18.17 & 0.19 & 15.89 & 0.12 &  \\
447 & 8 59 7.74 & -47 30 43.9 & 19.16 & 0.12 & 16.67 & 0.08 & 15.47 & 0.08 &  \\
448 & 8 59 7.82 & -47 30 58.2 & 18.23 & 0.09 & 16.13 & 0.07 & 15.09 & 0.08 &  \\
449 & 8 59 7.83 & -47 30 39.8 & \nodata & \nodata & \nodata & \nodata & 17.24 & 0.19 &  \\
450 & 8 59 7.84 & -47 30 18.2 & \nodata & \nodata & 16.52 & 0.09 & 13.98 & 0.05 &  \\
451 & 8 59 7.85 & -47 30 23.9 & 18.44 & 0.09 & 15.95 & 0.06 & 14.65 & 0.06 &  \\
452 & 8 59 7.87 & -47 31 0.4 & 16.68 & 0.04 & 14.38 & 0.03 & 13.07 & 0.03 &  \\
453 & 8 59 7.88 & -47 30 44.8 & \nodata & \nodata & 18.08 & 0.17 & 16.83 & 0.16 &  \\
454 & 8 59 7.90 & -47 30 35.2 & 19.97 & 0.18 & 17.32 & 0.11 & 15.88 & 0.10 &  \\
455 & 8 59 7.94 & -47 30 25.8 & 17.22 & 0.05 & 14.57 & 0.03 & 13.02 & 0.03 &  \\
456 & 8 59 7.95 & -47 30 33.6 & 15.87 & 0.03 & 12.89 & 0.02 & 10.90 & 0.01 & e \\
457 & 8 59 7.98 & -47 30 37.3 & \nodata & \nodata & \nodata & \nodata & 16.95 & 0.18 &  \\
458 & 8 59 7.99 & -47 30 38.4 & 17.39 & 0.05 & 14.78 & 0.04 & 13.37 & 0.03 &  \\
459 & 8 59 7.99 & -47 30 35.8 & 19.50 & 0.15 & 16.19 & 0.07 & 13.95 & 0.04 & e \\
460 & 8 59 7.99 & -47 30 42.7 & 19.75 & 0.17 & 17.24 & 0.11 & 15.81 & 0.10 &  \\
461 & 8 59 8.00 & -47 30 35.4 & \nodata & \nodata & \nodata & \nodata & 16.41 & 0.14 &  \\
462 & 8 59 8.00 & -47 30 50.3 & 17.30 & 0.05 & 14.96 & 0.04 & 13.72 & 0.04 &  \\
463 & 8 59 8.02 & -47 30 54.0 & \nodata & \nodata & 17.67 & 0.15 & 16.35 & 0.14 &  \\
464 & 8 59 8.03 & -47 30 47.4 & 18.06 & 0.07 & 15.38 & 0.05 & 13.78 & 0.04 &  \\
465 & 8 59 8.04 & -47 30 33.7 & \nodata & \nodata & 17.68 & 0.14 & 16.09 & 0.12 &  \\
466 & 8 59 8.06 & -47 30 47.2 & 17.65 & 0.06 & 15.06 & 0.04 & 13.46 & 0.04 & e \\
467 & 8 59 8.06 & -47 31 6.3 & \nodata & \nodata & \nodata & \nodata & 16.73 & 0.19 &  \\
468 & 8 59 8.07 & -47 30 25.3 & 18.33 & 0.09 & 15.66 & 0.06 & 14.22 & 0.05 &  \\
469 & 8 59 8.08 & -47 30 38.8 & 17.85 & 0.07 & 15.46 & 0.05 & 14.13 & 0.05 &  \\
470 & 8 59 8.09 & -47 30 43.8 & \nodata & \nodata & \nodata & \nodata & 17.03 & 0.18 &  \\
471 & 8 59 8.17 & -47 30 46.6 & 18.53 & 0.09 & 16.18 & 0.07 & 14.35 & 0.05 & e \\
472 & 8 59 8.18 & -47 30 51.4 & 17.98 & 0.08 & 16.22 & 0.07 & 14.42 & 0.06 & p \\
473 & 8 59 8.19 & -47 30 51.4 & \nodata & \nodata & 16.22 & 0.07 & \nodata & \nodata &  \\
474 & 8 59 8.24 & -47 30 18.8 & \nodata & \nodata & \nodata & \nodata & 15.87 & 0.12 &  \\
475 & 8 59 8.27 & -47 30 39.1 & \nodata & \nodata & 17.81 & 0.15 & 16.15 & 0.12 &  \\
476 & 8 59 8.30 & -47 30 33.9 & \nodata & \nodata & \nodata & \nodata & 17.09 & 0.19 &  \\
477 & 8 59 8.37 & -47 30 46.4 & 18.81 & 0.11 & 16.14 & 0.07 & 14.23 & 0.05 & e \\
478 & 8 59 8.39 & -47 30 17.3 & \nodata & \nodata & 17.34 & 0.14 & 15.96 & 0.13 &  \\
479 & 8 59 8.45 & -47 30 29.4 & 17.30 & 0.05 & 16.36 & 0.08 & 15.75 & 0.11 & x \\
480 & 8 59 8.46 & -47 30 47.1 & \nodata & \nodata & 17.40 & 0.15 & 16.21 & 0.14 &  \\
481 & 8 59 8.48 & -47 30 49.0 & \nodata & \nodata & 16.63 & 0.10 & \nodata & \nodata &  \\
482 & 8 59 8.49 & -47 30 27.6 & \nodata & \nodata & \nodata & \nodata & 15.78 & 0.11 &  \\
483 & 8 59 8.50 & -47 30 49.5 & \nodata & \nodata & \nodata & \nodata & 15.65 & 0.11 &  \\
\enddata
\tablecomments{In the Notes column, `e' refers to those sources with an
infrared excess, `p' to protostars, which are sources with an excess
greater than of that expected of a reddened T Tauri stars, and 'x' to
sources that have $J-H < 1$ and whose photometry is incorrect, for reasons
described in the text.  Units of right ascension are hours, minutes and
seconds, and unites of declination are degrees, arcminutes, and arcseconds.
Units of $J$, $J_{\rm err}$ $H$, $H_{\rm err}$ $K_s$ $(K_s)_{\rm err}$ are
magnitudes.  Table~\ref{src-list} is published in its entirety in the
electronic edition of the Astronomical Journal.   A portion is shown here
for guidance regarding its form and content.}
\label{src-list}
\end{deluxetable}

